Privacy-preserving Cloud-based DNN Inference

Deep learning as a service (DLaaS) has been intensively studied to facilitate the wider deployment of the emerging deep learning applications. However, DLaaS may compromise the privacy of both clients and cloud servers. Although some privacy preserving deep neural network (DNN) based inference techniques have been proposed by composing cryptographic primitives, the challenges on computational efficiency have not been well-addressed due to the complexity of DNN models and expensive cryptographic primitives. In this paper, we propose a novel privacy preserving cloud-based DNN inference framework (namely, "PROUD"), which greatly improves the computational efficiency. Finally, we conduct extensive experiments on two commonly-used datasets to validate both effectiveness and efficiency for the PROUD, which also outperforms the state-of-the-art techniques.

==> analysis.tex <==
\begin{theorem}
PROUD does not reveal any private information in semi-honest adversarial model.
\end{theorem}

%\begin{proof}
\noindent\textbf{Proof.} Considering PROUD consists of two subprotocols: 1) PolyF, and 2) MatF. Then, we will first analyze the security of two subprotocols, respectively. 

Recall that the input of PolyF is the encrypted intermediate ciphertext, which can be polynomially simulated by the server using the client's public key $pk$. Then, the server locally performs the computation of approximation with the client's public key and the additive property of the homomorphic cryptosystem. It does not leak any information (e.g., weight parameter) to the client. Thus, PolyF is secure. 

Similarly, MatF is locally executed by the server with the client's public key $pk$. It will not leak private information. 

%also based on the homormophic cryptosystem (the encoding can be viewed as the add-on in the encryption). The computation will not leakage the information of the encrypted data. 
Finally, the client receives the encrypted matrix computation result and decrypts it using $sk$. Again, the received ciphertext (of the result) from the protocol can be polynomially simulated by encrypting the final result using its public key $pk$. Per the composition theorem \cite{goldreich1998secure}, PROUD does not reveal any private information.  \hfill $\boxdot$


